DORY: Automatic End-to-End Deployment of Real-World DNNs on Low-Cost IoT MCUs

The deployment of Deep Neural Networks (DNNs) on end-nodes at the extreme edge of the Internet-of-Things is a critical enabler to support pervasive Deep Learning-enhanced applications. Low-Cost MCU-based end-nodes have limited on-chip memory and often replace caches with scratchpads, to reduce area overheads and increase energy efficiency -- requiring explicit DMA-based memory transfers between different levels of the memory hierarchy. Mapping modern DNNs on these systems requires aggressive topology-dependent tiling and double-buffering. In this work, we propose DORY (Deployment Oriented to memoRY) - an automatic tool to deploy DNNs on low cost MCUs with typically less than 1MB of on-chip SRAM memory. DORY abstracts tiling as a Constraint Programming (CP) problem: it maximizes L1 memory utilization under the topological constraints imposed by each DNN layer. Then, it generates ANSI C code to orchestrate off- and on-chip transfers and computation phases. Furthermore, to maximize speed, DORY augments the CP formulation with heuristics promoting performance-effective tile sizes. As a case study for DORY, we target GreenWaves Technologies GAP8, one of the most advanced parallel ultra-low power MCU-class devices on the market. On this device, DORY achieves up to 2.5x better MAC/cycle than the GreenWaves proprietary software solution and 18.1x better than the state-of-the-art result on an STM32-F746 MCU on single layers. Using our tool, GAP-8 can perform end-to-end inference of a 1.0-MobileNet-128 network consuming just 63 pJ/MAC on average @ 4.3 fps - 15.4x better than an STM32-F746. We release all our developments - the DORY framework, the optimized backend kernels, and the related heuristics - as open-source software.

==> bibl_old.tex <==
\begin{thebibliography}{10}
\providecommand{\url}[1]{#1}
\csname url@samestyle\endcsname
\providecommand{\newblock}{\relax}
\providecommand{\bibinfo}[2]{#2}
\providecommand{\BIBentrySTDinterwordspacing}{\spaceskip=0pt\relax}
\providecommand{\BIBentryALTinterwordstretchfactor}{4}
\providecommand{\BIBentryALTinterwordspacing}{\spaceskip=\fontdimen2\font plus
\BIBentryALTinterwordstretchfactor\fontdimen3\font minus
  \fontdimen4\font\relax}
\providecommand{\BIBforeignlanguage}[2]{{%
\expandafter\ifx\csname l@#1\endcsname\relax
\typeout{** WARNING: IEEEtran.bst: No hyphenation pattern has been}%
\typeout{** loaded for the language `#1'. Using the pattern for}%
\typeout{** the default language instead.}%
\else
\language=\csname l@#1\endcsname
\fi
#2}}
\providecommand{\BIBdecl}{\relax}
\BIBdecl

\bibitem{MAHDAVINEJAD2018161}
M.~S. Mahdavinejad, M.~Rezvan, M.~Barekatain, P.~Adibi, P.~Barnaghi, and A.~P.
  Sheth, ``{{Machine learning for internet of things data analysis: a
  survey}},'' \emph{Digital Communications and Networks}, vol.~4, no.~3, pp.
  161 -- 175, 2018.

\bibitem{motlagh2017uav}
N.~H. Motlagh, M.~Bagaa, and T.~Taleb, ``{{UAV-based IoT platform: A crowd
  surveillance use case}},'' \emph{IEEE Communications Magazine}, vol.~55,
  no.~2, pp. 128--134, 2017.

\bibitem{zanghieri2019robust}
M.~Zanghieri, S.~Benatti, A.~Burrello, V.~Kartsch, F.~Conti, and L.~Benini,
  ``{{Robust Real-Time Embedded EMG Recognition Framework Using Temporal
  Convolutional Networks on a Multicore IoT Processor}},'' \emph{IEEE
  Transactions on Biomedical Circuits and Systems}, 2019.

\bibitem{elijah2018overview}
O.~Elijah, T.~A. Rahman, I.~Orikumhi, C.~Y. Leow, and M.~N. Hindia, ``{{An
  overview of Internet of Things (IoT) and data analytics in agriculture:
  Benefits and challenges}},'' \emph{IEEE Internet of Things Journal}, vol.~5,
  no.~5, pp. 3758--3773, 2018.

\bibitem{palossi201964mw}
D.~Palossi, A.~Loquercio, F.~Conti, E.~Flamand, D.~Scaramuzza, and L.~Benini,
  ``{{A 64mW DNN-based Visual Navigation Engine for Autonomous Nano-Drones}},''
  \emph{IEEE Internet of Things Journal}, 2019.

\bibitem{conti2017iot}
F.~Conti, R.~Schilling, P.~D. Schiavone, A.~Pullini, D.~Rossi, F.~K.
  G{\"u}rkaynak, M.~Muehlberghuber, M.~Gautschi, I.~Loi, G.~Haugou
  \emph{et~al.}, ``{{An IoT Endpoint System-on-Chip for Secure and
  Energy-Efficient Near-Sensor Analytics}},'' \emph{IEEE Transactions on
  Circuits and Systems I: Regular Papers}, vol.~64, no.~9, pp. 2481--2494,
  2017.

\bibitem{conti2020memory}
F.~Conti, M.~Rusci, and L.~Benini, ``{{The Memory Challenge in Ultra-Low Power
  Deep Learning}},'' in \emph{NANO-CHIPS 2030}.\hskip 1em plus 0.5em minus
  0.4em\relax Springer, 2020, pp. 323--349.

\bibitem{gao2018ifq}
H.~Gao, W.~Tao, D.~Wen, T.-W. Chen, K.~Osa, and M.~Kato, ``{{Ifq-net:
  Integrated fixed-point quantization networks for embedded vision}},'' in
  \emph{Proceedings of the IEEE Conference on Computer Vision and Pattern
  Recognition Workshops}, 2018, pp. 607--615.

\bibitem{7551407}
Y.~{Chen}, J.~{Emer}, and V.~{Sze}, ``{{Eyeriss: A Spatial Architecture for
  Energy-Efficient Dataflow for Convolutional Neural Networks}},'' in
  \emph{2016 ACM/IEEE 43rd Annual International Symposium on Computer
  Architecture (ISCA)}, 2016, pp. 367--379.

\bibitem{7092475}
F.~{Conti} and L.~{Benini}, ``{{A Ultra-Low-Energy Convolution Engine for Fast
  Brain-Inspired Vision in Multicore Clusters}},'' in \emph{2015 Design,
  Automation Test in Europe Conference Exhibition (DATE)}, 2015, pp. 683--688.

\bibitem{sze2017hardware}
V.~Sze, Y.-H. Chen, J.~Emer, A.~Suleiman, and Z.~Zhang, ``{{Hardware for
  machine learning: Challenges and opportunities}},'' in \emph{2017 IEEE Custom
  Integrated Circuits Conference (CICC)}.\hskip 1em plus 0.5em minus
  0.4em\relax IEEE, 2017, pp. 1--8.

\bibitem{garofalo2020xpulpnn}
A.~Garofalo, G.~Tagliavini, F.~Conti, D.~Rossi, and L.~Benini, ``{{XpulpNN:
  Accelerating Quantized Neural Networkson on RISC-V Processors Through ISA
  Extensions}},'' in \emph{To appear at Design, Automation and Test in Europe
  Conference (DATE) 2020}.\hskip 1em plus 0.5em minus 0.4em\relax IEEE, 2020.

\bibitem{7870349}
G.~{Desoli}, N.~{Chawla}, T.~{Boesch}, S.~{Singh}, E.~{Guidetti}, F.~{De
  Ambroggi}, T.~{Majo}, P.~{Zambotti}, M.~{Ayodhyawasi}, H.~{Singh}, and
  N.~{Aggarwal}, ``{{A 2.9TOPS/W deep convolutional neural network SoC in
  FD-SOI 28nm for intelligent embedded systems}},'' in \emph{2017 IEEE
  International Solid-State Circuits Conference (ISSCC)}, 2017.

\bibitem{garofalo2020pulp}
A.~Garofalo, M.~Rusci, F.~Conti, D.~Rossi, and L.~Benini, ``{{PULP-NN:
  Accelerating Quantized Neural Networks on Parallel Ultra-Low-Power RISC-V
  Processors}},'' \emph{Philosophical Transactions of the Royal Society A},
  vol. 378, no. 2164, p. 20190155, 2020.

\bibitem{conti2016pulp}
F.~Conti, D.~Rossi, A.~Pullini, I.~Loi, and L.~Benini, ``{{PULP: A Ultra-Low
  Power Parallel Accelerator for Energy-Efficient and Flexible Embedded
  Vision}},'' \emph{Journal of Signal Processing Systems}, vol.~84, no.~3, pp.
  339--354, 2016.

\bibitem{hyperram}
\BIBentryALTinterwordspacing
Cypress. (2019) {{Cypress DRAM}}. [Online]. Available:
  \url{https://www.cypress.com/products/hyperram-memory}
\BIBentrySTDinterwordspacing

\bibitem{saidi2013optimizing}
S.~Saidi, P.~Tendulkar, T.~Lepley, and O.~Maler, ``{{Optimizing two-dimensional
  DMA transfers for scratchpad Based MPSoCs platforms}},''
  \emph{Microprocessors and Microsystems}, vol.~37, no.~8, 2013.

\bibitem{tagliavini2015adrenaline}
G.~Tagliavini, G.~Haugou, A.~Marongiu, and L.~Benini, ``{{Adrenaline: An openvx
  environment to optimize embedded vision applications on many-core
  accelerators}},'' in \emph{2015 IEEE 9th International Symposium on Embedded
  Multicore/Many-core Systems-on-Chip}.\hskip 1em plus 0.5em minus 0.4em\relax
  IEEE, 2015, pp. 289--296.

\bibitem{cecconi2017optimal}
L.~Cecconi, S.~Smets, L.~Benini, and M.~Verhelst, ``{{Optimal tiling strategy
  for memory bandwidth reduction for cnns}},'' in \emph{International
  Conference on Advanced Concepts for Intelligent Vision Systems}.\hskip 1em
  plus 0.5em minus 0.4em\relax Springer, 2017, pp. 89--100.

\bibitem{peemen2013memory}
M.~Peemen, A.~A. Setio, B.~Mesman, and H.~Corporaal, ``{{Memory-centric
  accelerator design for convolutional neural networks}},'' in \emph{2013 IEEE
  31st International Conference on Computer Design (ICCD)}.\hskip 1em plus
  0.5em minus 0.4em\relax IEEE, 2013, pp. 13--19.

\bibitem{tf-micro}
\BIBentryALTinterwordspacing
M.~Abadi, A.~Agarwal, and P.~B. et~al., ``Tensorflow lite for
  microcontrollers,'' 2015, software available from tensorflow.org. [Online].
  Available: \url{https://www.tensorflow.org/lite/microcontrollers}
\BIBentrySTDinterwordspacing

\bibitem{CubeAI}
\BIBentryALTinterwordspacing
{{ST Microelectronics}}. (2017) {{X-CUBE-AI}}. [Online]. Available:
  \url{https://www.st.com/en/embedded-software/x-cube-ai.html}
\BIBentrySTDinterwordspacing

\bibitem{GWTAutotiler}
\BIBentryALTinterwordspacing
{{GreenWaves Technologies}}. (2019) {{GAP8 Auto-tiler}}. [Online]. Available:
  \url{https://greenwaves-technologies.com/manuals/BUILD/AUTOTILER/html/index.html}
\BIBentrySTDinterwordspacing

\bibitem{flamand2018gap}
E.~Flamand, D.~Rossi, F.~Conti, I.~Loi, A.~Pullini, F.~Rotenberg, and
  L.~Benini, ``{{GAP-8: A RISC-V SoC for AI at the Edge of the IoT}},'' in
  \emph{2018 IEEE 29th International Conference on Application-specific
  Systems, Architectures and Processors (ASAP)}.\hskip 1em plus 0.5em minus
  0.4em\relax IEEE, 2018, pp. 1--4.

\bibitem{howard2017mobilenets}
A.~G. Howard, M.~Zhu, B.~Chen, D.~Kalenichenko, W.~Wang, T.~Weyand,
  M.~Andreetto, and H.~Adam, ``{{MobileNets: Efficient Convolutional Neural
  Networks for Mobile Vision Applications}},'' 2017.

\bibitem{s2018mobilenetv2}
M.~Sandler, A.~Howard, M.~Zhu, A.~Zhmoginov, and L.-C. Chen, ``{{MobileNetV2:
  Inverted Residuals and Linear Bottlenecks}},'' 2018.

\bibitem{tan2019efficientnet}
M.~Tan and Q.~V. Le, ``{{Efficientnet: Rethinking model scaling for
  convolutional neural networks}},'' \emph{arXiv preprint arXiv:1905.11946},
  2019.

\bibitem{lin2020mcunet}
J.~Lin, W.-M. Chen, Y.~Lin, J.~Cohn, C.~Gan, and S.~Han, ``{{MCUNet: Tiny Deep
  Learning on IoT Devices}},'' 2020.

\bibitem{capotondi2020cmix}
A.~Capotondi, M.~Rusci, M.~Fariselli, and L.~Benini, ``{{CMix-NN: Mixed
  Low-Precision CNN Library for Memory-Constrained Edge Devices}},'' \emph{IEEE
  Transactions on Circuits and Systems II: Express Briefs}, 2020.

\bibitem{choi2018pact}
J.~Choi, Z.~Wang, S.~Venkataramani, P.~I.-J. Chuang, V.~Srinivasan, and
  K.~Gopalakrishnan, ``{{Pact: Parameterized Clipping Activation for Quantized
  Neural Networks}},'' \emph{arXiv preprint arXiv:1805.06085}, 2018.

\bibitem{lai2018cmsis}
L.~Lai, N.~Suda, and V.~Chandra, ``{{Cmsis-nn: Efficient neural network kernels
  for arm cortex-m cpus}},'' \emph{arXiv preprint arXiv:1801.06601}, 2018.

\bibitem{rusci2018work}
M.~Rusci, A.~Capotondi, F.~Conti, and L.~Benini, ``Work-in-progress: Quantized
  nns as the definitive solution for inference on low-power arm mcus?'' in
  \emph{2018 International Conference on Hardware/Software Codesign and System
  Synthesis (CODES+ ISSS)}.\hskip 1em plus 0.5em minus 0.4em\relax IEEE, 2018,
  pp. 1--2.

\bibitem{gautschi2017near}
M.~Gautschi, P.~D. Schiavone, A.~Traber, I.~Loi, A.~Pullini, D.~Rossi,
  E.~Flamand, F.~K. G{\"u}rkaynak, and L.~Benini, ``{{Near-threshold RISC-V
  core with DSP extensions for scalable IoT endpoint devices}},'' \emph{IEEE
  Transactions on Very Large Scale Integration (VLSI) Systems}, vol.~25,
  no.~10, pp. 2700--2713, 2017.

\bibitem{helium}
\BIBentryALTinterwordspacing
ARM. (2017) Arm helium. [Online]. Available:
  \url{https://www.arm.com/why-arm/technologies/helium}
\BIBentrySTDinterwordspacing

\bibitem{10.1145/3358198}
S.~Dave, Y.~Kim, S.~Avancha, K.~Lee, and A.~Shrivastava, ``{{DMazeRunner:
  Executing Perfectly Nested Loops on Dataflow Accelerators}},'' \emph{ACM
  Trans. Embed. Comput. Syst.}, vol.~18, Oct. 2019.

\bibitem{nxp}
\BIBentryALTinterwordspacing
NXP. Nxp lpc4300. [Online]. Available:
  \url{https://www.nxp.com/products/processors-and-microcontrollers/arm-microcontrollers/general-purpose-mcus/lpc4300-cortex-m4-m0}
\BIBentrySTDinterwordspacing

\bibitem{Larq}
L.~Geiger and P.~Team, ``{{Larq: An Open-Source Library for Training Binarized
  Neural Networks}},'' \emph{Journal of Open Source Software}, vol.~5, no.~45,
  p. 1746, Jan. 2020.

\bibitem{st-dual}
\BIBentryALTinterwordspacing
{{ST Microelectronics}}. {{STM32H7}}. [Online]. Available:
  \url{https://www.st.com/en/microcontrollers-microprocessors/stm32h7-series.html}
\BIBentrySTDinterwordspacing

\bibitem{uTensor}
\BIBentryALTinterwordspacing
{{Neil Tan et al.}} (2019) $\mu$tensor. [Online]. Available:
  \url{https://github.com/uTensor/uTensor}
\BIBentrySTDinterwordspacing

\bibitem{wang2020fann}
X.~Wang, M.~Magno, L.~Cavigelli, and L.~Benini, ``{{FANN-on-MCU: An Open-Source
  Toolkit for Energy-Efficient Neural Network Inference at the Edge of the
  Internet of Things}},'' \emph{IEEE Internet of Things Journal}, 2020.

\bibitem{conti2020nemo}
F.~Conti, ``{{Technical Report: NEMO DNN Quantization for Deployment Model}},''
  2020.

\bibitem{pullini2019mrwolf}
A.~{Pullini}, D.~{Rossi}, I.~{Loi}, G.~{Tagliavini}, and L.~{Benini},
  ``{{Mr.Wolf: An Energy-Precision Scalable Parallel Ultra Low Power SoC for
  IoT Edge Processing}},'' \emph{IEEE Journal of Solid-State Circuits},
  vol.~54, no.~7, pp. 1970--1981, 2019.

\bibitem{rahimi2011fully}
A.~Rahimi, I.~Loi, M.~R. Kakoee, and L.~Benini, ``{{A fully-synthesizable
  single-cycle interconnection network for shared-l1 processor clusters}},'' in
  \emph{2011 Design, Automation \& Test in Europe}.\hskip 1em plus 0.5em minus
  0.4em\relax IEEE, 2011, pp. 1--6.

\bibitem{rossi2014ultra}
D.~Rossi, I.~Loi, G.~Haugou, and L.~Benini, ``{{Ultra-low-latency lightweight
  DMA for tightly coupled multi-core clusters}},'' in \emph{Proceedings of the
  11th ACM Conference on Computing Frontiers}, 2014.

\bibitem{pullini2017mudma}
A.~Pullini, D.~Rossi, G.~Haugou, and L.~Benini, ``{{$\mu$DMA: An autonomous I/O
  subsystem for IoT end-nodes}},'' in \emph{2017 27th International Symposium
  on Power and Timing Modeling, Optimization and Simulation (PATMOS)}.\hskip
  1em plus 0.5em minus 0.4em\relax IEEE, 2017, pp. 1--8.

\end{thebibliography}


==> text/table2.tex <==
\begin{table}[t]
\caption{Analysis in terms of complexity, memory footprint, and latency of MobileNet-v1 and MobileNet-v2.}
\label{tab:M1_M2}
\footnotesize
\centering
\begin{tabular}{cccc}
\multicolumn{1}{c|}{}          & \multicolumn{1}{c|}{Mult-and-Acc.} & \multicolumn{1}{c|}{Parameters} & Cycles  \\ \hline \hline
\multicolumn{4}{c}{\textbf{MobileNet-v1} (width mult 1.0, input 128x128)}                                                                       \\ \hline 
\multicolumn{1}{c|}{Conv 1x1}      & \multicolumn{1}{c|}{96.05\%}       & \multicolumn{1}{c|}{74.61\%}    & 69.55\% \\ \hline
\multicolumn{1}{c|}{DwConv 3x3}   & \multicolumn{1}{c|}{3.06\%}        & \multicolumn{1}{c|}{1.06\%}     & 25.16\% \\ \hline
\multicolumn{1}{c|}{FC}        & \multicolumn{1}{c|}{0.18\%}        & \multicolumn{1}{c|}{24.33\%}    & 5.28\%  \\ \hline
\multicolumn{1}{c|}{Add}       & \multicolumn{3}{c}{-}                                               \\ \hline
\multicolumn{1}{c|}{Total} & \multicolumn{1}{c|}{186.4M}        & \multicolumn{1}{c|}{4.2M}       & 23.3M   \\ \hline \hline
\multicolumn{4}{c}{\textbf{MobileNet-v2} (width mult 1.0, input 128x128)}                                                                       \\ \hline
\multicolumn{1}{c|}{Conv 1x1}      & \multicolumn{1}{c|}{91.94\%}       & \multicolumn{1}{c|}{61.25\%}    & 54.84\% \\ \hline
\multicolumn{1}{c|}{DwConv 3x3}   & \multicolumn{1}{c|}{6.70\%}        & \multicolumn{1}{c|}{1.84\%}     & 36.09\% \\ \hline
\multicolumn{1}{c|}{FC}        & \multicolumn{1}{c|}{1.36\%}        & \multicolumn{1}{c|}{36.92\%}    & 8.37\%  \\ \hline
\multicolumn{1}{c|}{Add}       & \multicolumn{1}{c|}{-}         & \multicolumn{1}{c|}{-}      & 0.70\%  \\ \hline
\multicolumn{1}{c|}{Total} & \multicolumn{1}{c|}{100.1M}         & \multicolumn{1}{c|}{3.4M}       & 19.0M   \\ \hline
\end{tabular}
\vspace{-0.4cm}
\end{table}

==> text/table3.tex <==
\begin{table*}[t]
\caption{End-to-end execution of image recognition MobileNet-v1 and MobileNet-v2 on GAP8 and STM32H7 MCUs, using DORY, GWT Autotiler, and X-CUBE-AI. 
Abbreviations Param.: total number of parameters, Ms: Multiply-and-accumulates, GM: giga-Ms, lat.: latency, and E: energy. }
\label{tab:comparison}
\footnotesize
\centering
\renewcommand{\arraystretch}{1.3}
\begin{tabular}{lllllllllllll}
\multicolumn{1}{l|}{}              & \multicolumn{1}{l|}{Param.} & \multicolumn{1}{l|}{Ms}    & \multicolumn{1}{l|}{Cycles}  & \multicolumn{1}{l|}{M/cyc.} & \multicolumn{1}{l|}{GM/s/W} & \multicolumn{1}{l|}{GM/s} & \multicolumn{1}{l|}{lat. {[}ms{]}} & \multicolumn{1}{l|}{E {[}mJ{]}} & \multicolumn{1}{l|}{GM/s/W} & \multicolumn{1}{l|}{GM/s} & \multicolumn{1}{l|}{lat. {[}ms{]}} & E {[}mJ{]} \\ \hline \hline
\multicolumn{13}{c}{DORY @ GAP8}                                                                                                                                                                                                                                                                                                                                                                                    \\ \hline \hline
\multicolumn{5}{l|}{}       & \multicolumn{4}{c|}{Low energy 1V @ 100 MHZ}                                                                                       & \multicolumn{4}{c}{Low latency 1.15V @ 260 MHZ}                                                              \\ \hline
\multicolumn{1}{l|}{1.0-M.V1-128}  & \multicolumn{1}{l|}{4.2 M}  & \multicolumn{1}{l|}{186.4 M} & \multicolumn{1}{l|}{28.5 M}  & \multicolumn{1}{l|}{6.53}     & \multicolumn{1}{l|}{12.80}    & \multicolumn{1}{l|}{0.65}   & \multicolumn{1}{l|}{281.47}        & \multicolumn{1}{l|}{14.31}      & \multicolumn{1}{l|}{6.53}     & \multicolumn{1}{l|}{1.70}   & \multicolumn{1}{l|}{109.80}        & 28.79      \\ \hline
\multicolumn{1}{l|}{1.0-M.V2-128}  & \multicolumn{1}{l|}{3.47 M} & \multicolumn{1}{l|}{94.3 M}  & \multicolumn{1}{l|}{20.5 M}  & \multicolumn{1}{l|}{4.61}     & \multicolumn{1}{l|}{9.04}     & \multicolumn{1}{l|}{0.46}   & \multicolumn{1}{l|}{204.59}        & \multicolumn{1}{l|}{10.43}      & \multicolumn{1}{l|}{4.61}     & \multicolumn{1}{l|}{1.20}   & \multicolumn{1}{l|}{78.69}         & 20.63      \\ \hline \hline
\multicolumn{13}{c}{GWT AUTOTILER @ GAP8}                                                                                                                                                                                                                                                                                                                                                                           \\ \hline \hline
\multicolumn{5}{l|}{}        & \multicolumn{4}{c|}{Low energy 1V @ 100 MHZ}                                                                                       & \multicolumn{4}{c}{Low latency 1.15V @ 260 MHZ}                                                              \\ \hline
\multicolumn{1}{l|}{1.0-M.V1-128}  & \multicolumn{1}{l|}{4.2 M}  & \multicolumn{1}{l|}{186.4 M} & \multicolumn{1}{l|}{40.3 M}  & \multicolumn{1}{l|}{4.63}     & \multicolumn{1}{l|}{8.46}     & \multicolumn{1}{l|}{0.46}   & \multicolumn{1}{l|}{402.87}        & \multicolumn{1}{l|}{20.55}      & \multicolumn{1}{l|}{4.63}     & \multicolumn{1}{l|}{1.20}   & \multicolumn{1}{l|}{154.95}        & 40.63      \\ \hline \hline
\multicolumn{13}{c}{X-CUBE-AI FITTING 2MB ROM 512 kB R/W MEMORY @ STM32H7}                                                                                                                                                                                                                                                                                                                                          \\ \hline \hline
\multicolumn{1}{l|}{0.25-M.V1-128} & \multicolumn{1}{l|}{0.5 M}  & \multicolumn{1}{l|}{13.5 M}  & \multicolumn{1}{l|}{26.0 M}  & \multicolumn{1}{l|}{0.52}     & \multicolumn{1}{l|}{1.07}     & \multicolumn{1}{l|}{0.25}   & \multicolumn{1}{l|}{51.14}         & \multicolumn{1}{l|}{12.67}      & \multicolumn{1}{l|}{n.a.}     & \multicolumn{1}{l|}{n.a.}   & \multicolumn{1}{l|}{n.a.}          & n.a.       \\ \hline
\multicolumn{1}{l|}{0.5-M.V1-192}  & \multicolumn{1}{l|}{1.37 M} & \multicolumn{1}{l|}{109.5 M} & \multicolumn{1}{l|}{212.3 M} & \multicolumn{1}{l|}{0.52}     & \multicolumn{1}{l|}{1.06}     & \multicolumn{1}{l|}{0.25}   & \multicolumn{1}{l|}{442.27}        & \multicolumn{1}{l|}{103.49}     & \multicolumn{1}{l|}{n.a.}     & \multicolumn{1}{l|}{n.a.}   & \multicolumn{1}{l|}{n.a.}          & n.a.       \\ \hline
\end{tabular}
\vspace{-0.3cm}
\end{table*}

==> text/table_DORY_API.tex <==
\begin{table*}
\centering
{\color{red}
\caption{Deployment of DORY on two example platforms, an STM32F7 and the GAP8 previously analysed.}
\vspace{-0.3cm} 
\label{tab:DORY_APIs}
\begin{tabular}{l|l|l|l}
        & \textbf{Heuristics}                                          & \textbf{Mem. API}                                                                                                                  & \textbf{Backend}                                                                                                                   \\ \hline
DORY    & \begin{tabular}[c]{@{}l@{}}C1\\ C2\\ …\end{tabular} & \begin{tabular}[c]{@{}l@{}}\texttt{DORY\_dma\_memcpy\_3d();}\\ \texttt{DORY\_dma\_memcpy\_2d();}\\ \texttt{DORY\_dma\_wait();}\end{tabular}                           & \begin{tabular}[c]{@{}l@{}}\texttt{DORY\_conv();}\\ \texttt{DORY\_conv\_dw();}\\ …\end{tabular}                                             \\ \hline \hline
\multicolumn{4}{l}{\textbf{DORY deployments}}\\\hline\hline
STM32F7 &        \begin{tabular}[c]{@{}l@{}}   $\mathcal{H}_{i2c} = C_y^t$ \\   $    \mathcal{H}_{mm\_w} = (w_{y}^t-1)\,\mathrm{mod}\,2\;;\;$\\$\mathcal{H}_{mm\_ch} = (C_{y}^t-1)\,\mathrm{mod}\,4 $\end{tabular}                                               & \begin{tabular}[c]{@{}l@{}}\texttt{HAL\_MDMA\_Start\_IT();}\\\texttt{HAL\_MDMA\_RegisterCallback();}\end{tabular} & \begin{tabular}[c]{@{}l@{}}\texttt{arm\_convolve\_HWC\_q7\_fast();}\\ \texttt{arm\_depthwise\_separable\_conv\_HWC\_q7();}\\ …\end{tabular} \\ \hline


GAP8    &      \begin{tabular}[c]{@{}l@{}}   $\mathcal{H}_{i2c} = C_y^t$ \\  $    \mathcal{H}_{par} = (h_{y}^t-1)\,\mathrm{mod}\,8
    $  \\ $    \mathcal{H}_{mm\_w} = (w_{y}^t-1)\,\mathrm{mod}\,2\;;\;$\\$\mathcal{H}_{mm\_ch} = (C_{y}^t-1)\,\mathrm{mod}\,4 $\end{tabular}                                                & \begin{tabular}[c]{@{}l@{}}\texttt{mchan\_transfer();}\\ \texttt{mchan\_barrier();}\end{tabular}                                                                  & \begin{tabular}[c]{@{}l@{}}\texttt{pulp\_nn\_conv();}\\ \texttt{pulp\_nn\_conv\_pointwise();}\\ …\end{tabular}                              \\ \hline
\end{tabular}
}
\end{table*}

